Named Entity Recognition with Partially Annotated Training Data

Supervised machine learning assumes the availability of fully-labeled data, but in many cases, such as low-resource languages, the only data available is partially annotated. We study the problem of Named Entity Recognition (NER) with partially annotated training data in which a fraction of the named entities are labeled, and all other tokens, entities or otherwise, are labeled as non-entity by default. In order to train on this noisy dataset, we need to distinguish between the true and false negatives. To this end, we introduce a constraint-driven iterative algorithm that learns to detect false negatives in the noisy set and downweigh them, resulting in a weighted training set. With this set, we train a weighted NER model. We evaluate our algorithm with weighted variants of neural and non-neural NER models on data in 8 languages from several language and script families, showing strong ability to learn from partial data. Finally, to show real-world efficacy, we evaluate on a Bengali NER corpus annotated by non-speakers, outperforming the prior state-of-the-art by over 5 points F1.

==> excised.tex <==
%Our method (Figure \ref{algorithm}) is best understood as an instantiation of the CODL framework \cite{ChangRaRo07} in the partially annotated NER scenario. CODL (short for Constraint Driven Learning) is an iterative process for semi-supervised learning that is related to self-training, but guides each iteration using knowledge-based constraints.\SC{Instead of talking about CoDL, talk about your algorithm.} \footnote{The original paper has a more detailed discussion on the distinction between CODL and self-training. \SC{You don't need to talk about this. It was a job of CoDL authors.}}

%Although our algorithm is based on CODL, we differ in several important ways. First, as is common in the semi-supervised tradition, CODL assumes a small amount of fully supervised data to train an initial model. In our scenario, this is not available, and we have only partially annotated data (although it is easy to incorporate fully annotated data). Our experiments show that a good initialization is helpful, but not strictly necessary.


%gives low weights to all predicted positives in $N$. Recall that our approach is to weight tokens according to confidence in labeling. If our algorithm has decided that a token in $N$ is positive, we take this to mean that the true label is positive, and it is therefore mislabeled. This token will get a low weight. All other tokens in $N$ are weighted proportional to the classifier confidence. 



% We are left with set $P$, unchanged from before, and set $N$, with all mislabeled entities (and some innocent bystanders) removed. Further, all other tokens in $N$ are weighted by prediction confidence. We rescale the weights so the entity ratio is roughly balanced, and then train a weighted multi-class classifier.






% \swm{=== Maybe don't need the below ====}


% The first step is to find all the missing entities in the training data. The algorithm iteratively runs two steps: 1) train and predict and 2) infer labels and weights.

% In the first step, we train a classifier on the current (weighted) dataset, and make predictions on that same dataset.

% In the second step, we run inference with an ILP in order to get new labels and weights on the dataset for the next round.

% The first step is self-explanatory, but the second step (inference) requires a little more explanation. Recall that the purpose of this algorithm is to add more entities. To that end, there is a constraint that requires that a certain number of tokens are classified as entity. This number grows at each iteration until it reaches a known golden entity ratio. We make the key assumption that we know roughly *how many* entities should be present in any given dataset. (We relax this assumption later on). \CT{Not sure how general do we want to present the framework. The "entity ratio" is specific to NER. If we decided to be task-agnostic here, maybe use "positive ratio" instead?}

% While the entity ratio constraint is the most important, there are other constraints also, intended to increase the precision of the new labeling. These can be different depending on the language or domain. For example, in English we may include a soft constraint that entities must be capitalized.

% So far, we have modified the labeling on the dataset by adding more entities. The next step is to modify the weighting.

% \CT{More explanation is needed for this paragraph. e.g., ILP is not mentioned before.} If it is a member of P it gets weight 1. If the ILP labeled it as positive, this means is has top-ranked confidence so it gets weight 1. If the ILP labeled it as negative: a) and the classifier originally labeled as negative, it is assigned weight corresponding to prediction confidence b) but the classifier originally labeled as positive, then it gets weight 0.


% \swm{======= What follows is old ========}

% Like standard self-training we iteratively train on our train set ($T$ in the figure), and then predict on it, correcting and selecting predictions to improve training on the next round. Armed with the intuition that removing too many noisy instances is better than removing too few, at each round we bias the model towards predicting positives, by scaling the weights of the train set (using the technique in Section \ref{sec:entityratio}) before training.\footnote{In our experiments, we set the entity ratio to twice the true ratio.}


% Since the goal is just to flag and remove entities, regardless of label, we map our multiclass training data into a binary label space, where all entities (Person, Organization, etc) are treated as Positive, and all non-entities are treated as Negative (line 3).  In theory, using binary labels should give higher scores than multiclass labels because we need not worry about labeling mistakes between types. We keep track of original labels, and unmask set $P$ (line 11) at the end before training the final model.



% %\SC{There is no point in talking about the value of entity ratio here. Maybe it would make more sense in Section \ref{sec:entityratio} or as a footnote.}

% We formulate the problem of selecting instances for training (line 8) as constrained optimization, using an Integer Linear Program (ILP), the details of which are given in Section \ref{sec:ilp}. This allows us to enforce language- or task-specific constraints based on classifier predictions to improve performance. One important constraint (Eqn. \ref{posconstraint}) governs how many positives are labeled at each round. This number starts at $|P|$ and is increased by a $\Delta$ value\footnote{$\Delta$ is related to how much we trust the ranking induced by prediction confidences. If we believed the ranking was perfect, we could take as many positives as we wanted and be finished in one round.} at each iteration, thereby improving recall. Positive instances are chosen in two ways. First, all instances in $P$ are constrained to be labeled positive (Eqn. \ref{pconstraint}). Second, the objective function ensures that high-confidence positives will be chosen. The stopping condition is met when the number of required positive instances equals the number of true positive instances, which we can calculate assuming knowledge of the entity ratio.

% % swm: true, but not all that useful, or important.
% %Unlike standard self-training, the additional high confidence positives are not permanently added to $P$. We train on them as positives in the next round, but it is possible they will be classified as negative in later rounds as the classifier improves.

% After the ILP has selected predictions, we assign weights to each instance in preparation for training the next round. The decision process for an instance is as follows:
% \begin{itemize}
%  \item If it is a member of $P$ it gets weight 1.
% \item  If the ILP labeled it positive, this means it has top-ranked confidence, so it gets weight 1.
% \item If the ILP labeled it as negative:
% \begin{itemize}
% \item And the classifier originally labeled as negative, it is assigned weight corresponding to prediction confidence.
% \item But the classifier originally labeled as positive, then it gets weight 0.
% \end{itemize}
% \end{itemize}

%  With these new labels, and new weights, we start the next iteration.


% \begin{figure}
% \begin{algorithmic}[1]
% %\Define
% %\Statex 1, 0: Positive and negative labels
% \Require
% \Statex $P$ : positive tokens
% \Statex $N$ : noisy negative tokens
% %\Statex $U: \{(t_j)\}_{j=1}^M$
% %\Statex $h$: a heuristic weighting function (\S \ref{sec:heuristics})
% %\Statex $\delta$ = increment value for $b$
% %\Statex $b^*$ = known gold entity ratio for $P+U$
% \Statex
% \State $T = N \cup P$ \Comment Training set
% \State Initialize $T$ with weights \Comment \S~\ref{sec:weightingschemes}
% %\State Convert $T$ to binary labeling
% \While{stopping condition not met}
% 	%\State Rescale $T$ (favor positives) \Comment \S~\ref{sec:entityratio}
%   \State Train on $T$ %\Comment Weighted training
% 	\State Predict on $T$
%   \State Correct and select with constraints, rescale \Comment \S~\ref{sec:ilp}
%     %\State Add top $k_t$ positives to $P$
%     %\State All other positives get weight 0
%     %\State Assign weights to negatives acc. to conf.
%     %\State $k_{t+1} = k_t + \delta$
% \EndWhile
% %\State Set $P$ to the original set, multiclass
% \State Predicted positives in $N$ get weight 0 \Comment 0-weight
% %\State Assign weights to other negatives acc. to conf.
% %\State Revert $T$ back to multiclass
% %\State Rescale $T$ (balanced)
% %\State Train on $T$
% %\State Predict on Test \Comment Multiclass predictions
% \end{algorithmic}
% \caption{Constrained Driven Learning Partial (CODL-P) algorithm. The core of the algorithm is in the while loop, which iterates over training on $T$, predicting on $T$ and correcting those predictions. Before training, we always rescale the weights on $N$ so that the model will overpredict entities in the next round.}
% \label{algorithm}
% \end{figure}


% \section{ILP in the Multiclass Case}
% The ILP for the multiclass case is found in Figure \ref{multiclassilp}.

% \begin{figure}
% \begin{equation*}
% \begin{aligned}
% & \underset{\textbf{y}}{\text{max}} & & \sum_i \sum_t C_{t_B} y_{t_Bi} + C_{t_I} y_{t_Ii}  \\
% & \text{s.t.} & & \forall i, y_Oi + \sum_t y_{t_Bi} + y_{t_Ii} = 1 \\
% & & & b-\delta \leq 1 - \sum_i y_{Oi} / N \leq b+\delta \\
% & & & \forall i,  \text{isPunc}(x_i) \vee \text{isNum}(x_i), y_{Oi} = 1,  \\
% &&& \forall t \in T\cup O, \forall w \in W,  \\
% &&& ~~~~~|S_w| a_t + \sum_{i \in S_w} [ y_{t_Bi} + y_{t_Ii} ] \geq \alpha |S_w| \\
% & & & ~~~~~\sum_{t\in T} a_t=|T| \\
% & & &  \forall i, \forall t\in T, y_{t_Bi} + y_{t_Ii} + \sum_{t' \in T_I/t_I} y_{t'(i+1)} \leq 1 \\
% & & &  \forall i, y_{Oi} + y_{T_I(i+1)} \leq 1 \\
% \end{aligned}
% \end{equation*}
% \caption{ILP for the multiclass case. Parameters are $b$, $\delta$, $\alpha$. $C_0$ and $C_1$ are probabilities from the classifier of class 0 and class 1.}
% \label{multiclassilp}
% \end{figure}

% $T$ is the set of all classes (PER, ORG, LOC), not including the O tag. $T_B$ is the set of all tags, but with the $B-$ prefix. $t_B$ is a specific tag with $B-$ prefix. $W$ is the set of unique word forms in the corpus. $S_w$ is the set of occurrences of word form $w$. The last two constraints enforce rules from the BIO scheme (the token before an I- tag must share the same class, and I cannot come after B).

%\dan{took out "artificially perturbed"; it's a negative statement that is not completely correct; we just drop some of the labels to test the algorithm, not touching the data. I did not find if it's described this way elsewhere, but if it does please correct it.}

%\SC{otherwise, are unlabeled or labeled as non-entities}
% swm: not sure I understand this comment.
% \SC{"labeled as non-entities" might be a bit confusing. They were actually left unlabeled and you assumed that they should be treated as non-entities.}

% \SC{I wouldn't use the term "dataset cleaning"}
% swm: OK. I'm going with denoising... how's that? Or, making the data usable.
%\SC{words like these make it sound like a data mining paper instead of an NLP paper and, to some extent, trivializes the problem. There is much more to the problem than "cleaning"....one of the two classes is missing and you need to use domain knowledge to identify examples from both classes and then train a classifier. This is much more than what data cleaning people do. Can we rephrase without using any of these words? If it is absolutely necessary, reduce their frequencies and not use them in prominent places? }


%%%---------- close: ilp


%Further, we show that a good initialization can improve performance significantly.

%SC{"for segregating true entities and non-entities out of this noisy training data" instead of "cleaning partially annotated training data"} 
% swm: I don't like segregating because it suggests hard decisions. I make soft decisions.
%\SC{Makes sense but I would recommend coming up with another alternative for "cleaning"}

% We introduce an iterative self-training algorithm called Constrained Binary Learning (CBL) that uses knowledge-based constraints to guide learning, similar to Constraint Driven Learning \cite{ChangRaRo07}.

%As we seek these mislabeled entities for removal, we make the observation that there is an asymmetric cost to these predictions. If we remove too few mislabeled entities, then we still have noise, which is costly. But if we bias the model towards predicting \SC{don't talk about prediction yet as you haven't explained that yet }and removing more entities, we risk only the loss of potentially redundant non-entity tokens.

%\SC{In the previous para you are assuming that the reader understands that you are going to identify true-entities and throw them away (instead of putting them in $P$). You need to either talk about that before this paragraph or not bring it up here.}

% \begin{figure}[t]
% \centering
% \begin{tabular}{l}
% \fbox{\begin{minipage}{19em}
% \raggedright
% New York attack underlines [Central Asia]\textsubscript{LOC} as a growing source of terrorism
% \end{minipage}}\\
% \end{tabular}
% \caption{This box shows a partially annotated sentence. There are two locations, \textit{New York} and \textit{Central Asia}, but only one is labeled.}
% \label{example}
% \end{figure}


%To the best of our knowledge, we are the first work that addresses the problem of partial annotation for NER in the situation in which there are no reliable examples of non-entities.

% \subsection{Self-training for NER}
% Self training to improve NER has also been done before:

% \cite{tackstrom2012nudging} does self-training for NER, using the analogy of multilingual processing as domain adaptation. They weight the target-language instances according to the confidence of the original classifier. Filter low-confidence predictions.

% \cite{angeli2015bootstrapped} do KBP relation extraction via bootstrapping or self-training. Interesting note: they have high-recall extractors, use these to gather high-probability negative examples. They always train on the original labeled set.

% Bootstrapping from Wikipedia annotations \cite{PZMNKJ17}.

% \subsection{Low resource work?}

% \cite{wang2013cross} project annotations across parallel text, but train with a generalized expectation framework that treats a distribution over tags as a constraint on the learning problem. These label distributions come from the projections over the bitext. They show that this framework is much better than the classic project-then-train approach, even when hard confidences are projected.

% \cite{wang2013cross} draw heavily from \cite{mann2010generalized}, introduces the Generalized Expectation (GE) criteria framework. The running example in \cite{mann2010generalized} is label regularization, where the desired output label proportions are known, and used as constraints on the learning.


% Bootstrapping for domain adaptation \cite{sun2011cross}. They start with a source model and bootstrap using confidence, as well as several other heuristics for selection. See also \cite{wu2009domain}.

% Constrained NER with an ILP \cite{che2013named}. They use bitext to impose constraints.

% Graham Neubig ``pointwise classifier'', just refers to classifying in a non-sequential fashion. Each word is a point.


% \cite{clark2003bootstrapping} bootstrapping for POS.
% \cite{petrov2010uptraining}. Uptraining for question parsing.

% \cite{mohit2011recall} does NER on Arabic Wikipedia.
%%%---------- close: relatedwork

%  \SC{scaled to be between 0 and 1?}
% swm: no. We use raw confidence scores from the classifier. They just need to be comparable. we will rescale them as part of the balancing.

%Ultimately, we send the original multiclass partially annotated dataset along with final weights $V$ to a standard weighted NER classifier to learn a model. No weights are needed at test time.


%\subsection{NER-Specific Details}
% So far, we have given a high-level view of the algorithm. In this section, we will give more low-level details, especially as they relate to the specific problem of NER. The most tricky part in the above algorithm is the inference step (line 6), which we address using a constrained Integer Linear Program (ILP) and describe in this section. However, the constraints are based on a value we call the \textit{entity ratio}. First, we describe the entity ratio, then we describe the constraints and stopping condition of the algorithm.

% swm: these were good comments.
%\SC{You need a few statements about why the reader needs to know about entity ratio. 




%\swm{At this point, a reader understands the overall strategy (data denoising), the general algorithm (Fig 2), and hopefully the constraints that we use. We have only mentioned the entity ratio, but have not fully described it. Also, it is not clear what changes in each iteration of the loop. This needs to be made clear, or the stopping condition.}


%\swm{stopping condition} 


% \begin{itemize}
%  \item If it is a member of $P$ it gets weight 1.
% \item  If the ILP labeled it positive, this means it has top-ranked confidence, so it gets weight 1.
% \item If the ILP labeled it as negative:
% \begin{itemize}
% \item And the classifier originally labeled as negative, it is assigned weight corresponding to prediction confidence.
% \item But the classifier originally labeled as positive, then it gets weight 0.
% \end{itemize}
% \end{itemize}


% \subsection{Self-training for NER}
% Self training to improve NER has also been done before:

% \cite{tackstrom2012nudging} does self-training for NER, using the analogy of multilingual processing as domain adaptation. They weight the target-language instances according to the confidence of the original classifier. Filter low-confidence predictions.

% \cite{angeli2015bootstrapped} do KBP relation extraction via bootstrapping or self-training. Interesting note: they have high-recall extractors, use these to gather high-probability negative examples. They always train on the original labeled set.

% Bootstrapping from Wikipedia annotations \cite{PZMNKJ17}.

% \subsection{Low resource work?}

% \cite{wang2013cross} project annotations across parallel text, but train with a generalized expectation framework that treats a distribution over tags as a constraint on the learning problem. These label distributions come from the projections over the bitext. They show that this framework is much better than the classic project-then-train approach, even when hard confidences are projected.

% \cite{wang2013cross} draw heavily from \cite{mann2010generalized}, introduces the Generalized Expectation (GE) criteria framework. The running example in \cite{mann2010generalized} is label regularization, where the desired output label proportions are known, and used as constraints on the learning.


% Bootstrapping for domain adaptation \cite{sun2011cross}. They start with a source model and bootstrap using confidence, as well as several other heuristics for selection. See also \cite{wu2009domain}.

% Constrained NER with an ILP \cite{che2013named}. They use bitext to impose constraints.

% Graham Neubig ``pointwise classifier'', just refers to classifying in a non-sequential fashion. Each word is a point.


% \cite{clark2003bootstrapping} bootstrapping for POS.
% \cite{petrov2010uptraining}. Uptraining for question parsing.

% \cite{mohit2011recall} does NER on Arabic Wikipedia.
%%%---------- close: relatedwork


% swm: I prefer "assigning" for two reasons: that also encompasses our weight guesses, and we don't exactly "learn" the weights. We learn a classifier that gives us weights.

%\SC{will it be correct to use tokens instead of elements here? That will clarify things}
% swm: this is still in the "slightly more general" section, so I wanted to avoid the use of "tokens"



% Gold & 90.8 & 72.5 & 82.5 & 82.6 & 67.2 & 53.4 & 74.4 & 74.4 & 80.3 & 75.1 \\
% \midrule
% Oracle Weighting & 83.7 & 65.7 & 76.2 & 76.4 & 54.3 & 42.0 & 64.2 & 56.3 & 68.5 & 65.2 \\
% \midrule
% Raw annotations & 57.4 & 39.5 & 52.2 & 50.4 & 32.1 & 35.1 & 40.5 & 33.3 & 46.2 & 43.0 \\
% Window only & 57.1 & 35.1 & 49.7 & 38.4 & 42.5 & 29.2 & 36.2 & 33.0 & 49.3 & 41.2 \\
% Frequency only & 70.2 & 48.0 & 62.3 & 67.4 & 44.3 & 37.1 & 54.7 & 54.9 & 57.9 & 55.2 \\
% Combined Weighting & 75.2 & 56.6 & 70.8 & 70.8 & 46.5 & \textbf{44.1} & 57.7 & 57.5 & 60.2 & 59.9 \\
% \midrule
% CBL-Raw & 74.7 & \textbf{63.0} & 68.7 & 67.0 & 45.0 & 37.8 & 57.0 & 50.6 & \textbf{67.9} & 59.0 \\
% CBL-Combined & \textbf{77.3} & 61.8 & \textbf{74.0} & \textbf{72.4} & \textbf{49.2} & 43.7 & \textbf{59.3} & \textbf{58.2} & 67.6 & \textbf{62.6} \\

%Raw annotations (BiLSTM, adam=0.001) & &&&& 37.4 & 34.7 & 36.0 & 48.4 &  \\
%Freq, b=0.1, BiLSTM & &&&& 31.7 & 32.3 & 38.2 & 42.8 \\
%Freq, b=0.2, BiLSTM & &&&& 35.6 & 33.0 & 36.3 & 42.8 \\
% Freq, sent BiLSTM-CRF &&&&& 38.2 & 35.8 & 43.6 & 53.9 & \\
%Freq, simple tok BiLSTM && 35.6 && 33.4 & 31.8 & 16.8 & 38.2 & 50.8 \\
%Freq, simple tok (no avg, b=0.01) BiLSTM && 42.4 & 56.8 & 49.3 & 36.5 & 26.7 & 41.1 & 48.5  &  \\

%Raw annotations (neural) & 63-68.9 & 35.1 &&  42.3 & 30.6 & 34.4 & 27.7 & 47.8 & \\
%Frequency (neural) & 72-74 &&&& 31.3 & 29 & 41.7 & 53.1 & \\

%Class weighting & 57.4 & 39.5 & 52.2 & 50.4 & 32.1 & 35.1 & 33.3 & 46.2 & 43.3 \\

  %~~- Window only & 57.1 & 35.1 & 49.7 & 38.4 & 42.5 & 29.2 & 33.0 & 49.3 & 41.8 \\
  %~~- Frequency only & 70.2 & 48.0 & 62.3 & 67.4 & 44.3 & 37.1 & 54.9 & 57.9 & 55.3 \\


%& BiLSTM & 69.7 & \textbf{65.9} & 73.3 & 57.7 & 41.0 & 36.4 & 48.3 & 62.4 & 56.8 \\
%\midrule
%Jiateng & -- & 57.8 & 72.4 & 71.3 & -- & -- & -- & -- & -- \\

%Gold (BERT) & & & & & 49.7 & 51.6 & 72.6 & 72.6 & \\
%Gold (BiLSTM-CRF, fasttext) & & & & & 55.7 & 48.0 & 62.9 & 66.2 & \\
%Gold (neural, fasttext) & 89.5 & 54.5 &  & 73.5 & 51.7 & 46.1 & 51.9 & 61.8 & \\
%Gold (neural, myvecs, crf) & 90.5? & 77.3(crf) & \\
%Gold (neural, myvecs, nocrf) & 89.5 & 75.4 & & 78.9 & 62.9 & 47.9 & 69.8 & 77.4 & \\


%& BiLSTM & 73.3 & 67.2 & 77.2 & 65.2 & 50.7 & 38.1 & 48.2 & 68.5 & 61.1 \\
%Oracle Weighting (BiLSTM) 
%Oracle Weighting sent (BiLSTM) & &&&& 40.7 & 36.0 & 45.0 & 54.4 & \\

%Raw annotations (BiLSTM-CRF, adam=0.01) & &&&& 30.5 & 26.2 & 38.6 & 55.4 & \\
%& BiLSTM-CRF & 58.9 & 58.7 & 61.9 & 58.4 & 35.7 & 36.4 & 43.3 & 57.2 & 51.3 \\


%In general, we are successful, with some notable exceptions. In German and Somali, where \textit{CBL-Raw} beat \textit{CBL-Combined}, it is because they are on opposite sides of the precision/recall tradeoff, and the more conservative \textit{CBL-Raw} strikes a better balance. In Hindi and Arabic, when the Oracle weighting is not the best, it is again because the Oracle weighting makes imbalanced predictions (high precision, low recall) and our methods make a better balance.

%By the same token, the notion of the gold entity ratio as stopping condition gives some control over the precision and recall of the final predictions. For example, to get a model with particularly high recall, you only need to set the ``gold'' entity ratio to be artificially high. 

%\textbf{Inconsistencies}~ There are 3 odd results, in need of explanation. First, why is \textit{CBL-Raw} the best for German only? As before, the precision/recall tradeoff is the explanation, where the Combined initialization favored recall, and the Raw favored precision. Although other languages had similar results, the Combined initialization for German lost too much precision.

%Second, why is the best score from Arabic from the Combined Weighting scheme? The answer is that the combined weighting scheme initialization, when predicting on train, has relatively poor recall (intermediate scores omitted for space). This means that each step included

%\CT{Can we say something about Arabic?}




% \subsubsection{Using a Neural Model}
% \label{sec:neural}
% Since the only explicit requirement CBL makes of an NER system is that it takes instance weights in training, we also experimented with a BiLSTM architecture modified to take instance weights in training. Most neural NER systems include a CRF layer on top of the BiLSTM \cite{Collobert2011NaturalLP,LBSKD16}, but as the loss is computed at the sentence level, it is non-trivial to incorporate token-level instance weights. Instead, we omitted the CRF layer and used cross-entropy loss at the token level. (We experimented with and without the CRF layer, we found that the performance changes little if we omit it. A similar conclusion can be found in \cite{LBSKD16}.)

% To incorporate the instance weights, we simply multiplied the token-level cross-entropy loss for each token $x_i$ by the instance weight $v_i$. If the instance weight is 1, then the loss is unchanged. If the instance weight is 0, the loss does not contribute to any model updates. In principle, values in between 0 and 1 should soften the impact of that loss. Instance weighting has been used in a similar fashion in neural models for machine translation \cite{wang2017instance} and dialogue \cite{lison2017not}.


%\[ \text{loss}(x_i) = v_i \cdot \sum_{c=1}^k -\mathbbm{1}[y_i = c] \log p(\hat{y}_i = c \mid x_i)] \]

%Where $y_i$ and $\hat{y_i}$ are gold and predicted labels, respectively. 

% In our experiments, we found that the basic intuitions of this paper held true with the neural model. Training on raw data led to high precision, low recall predictions. Training with Oracle weights improved performance significantly. Training with frequency-based weights improved somewhat over the baseline.

% However, many of the finer details did not transfer. In particular, we found that the neural network did not respond to instance weights in the same way the linear model did. For instance, although the neural model scored 47.3 on Raw annotations in Somali, it reached only 53.1 while using Frequency only as the weighing scheme. This is much lower than the performance of the linear model (57.9). This was mainly a problem of balance: the neural Frequency only output had high recall and low precision. In the linear model, we could control this balance by changing the entity ratio, but for the neural network, this was not the case. We leave exploration of this non-trivial problem to future work. 

% Instead, our main results compare with \cite{HedderichKl18}, which proposed a neural model for solving a similar problem.

%In the absence of such techniques, we would point out that we compare against \cite{HedderichKl18}, which uses a somewhat more natural method of dealing with annotation noise.

%You could then smooth into the \cite{HedderichKl18} model. Say they proposed a neural model for solving a similar problem and we compare with them.


%There could be multiple reasons for this behavior, including poor quality of word-embeddings, and small size of the training data. A more likely reason is that a linear model can use the entity ratio as a natural way to trade-off between precision and recall.

%Now you could talk about poor quality of  word-embeddings in low-resource languages. Then say that a more likely reason is that in linear models, changing entity ratio is a natural way to trade-off between P and R. On the other had, including token weights in this manner is not a natural fit for neural models. 

%However, many of the finer details did not transfer. In particular, we found that the neural network did not respond to instance weights in the same way the linear model did. Using the frequency weights improved performance over the baseline, but not as significantly as the linear model. For example, in Somali, the neural model achieved 47.3 on Raw annotations, but only 53.1 with Frequency only (compare with 57.9 from the linear model). This was mainly a problem of balance: the Frequency only output would have high recall and low precision. In the linear model, we could control this balance by changing the entity ratio,

%but in the neural model even vastly different entity ratios at train time did not impact scores at test time. 

%Since the main goal of this paper is to learn meaningful instance weights, we consider this a negative result, and chose not to run full experiments with the neural method. 




%We emphasize that despite the success of neural models in recent years, linear models still play an important role. Not only are they faster to train and test, but they also tend to work better in low-resource scenarios \cite{Koehn2017SixCF}, where high-quality data and embeddings may not be available.


%For example, CBL relies heavily on the fact that the scaling of the weights (the $\gamma$ parameter) impacts performance in a transparent and meaningful way. That is, if you want a higher entity ratio in test, simply set a higher entity ratio in train. It is this observation that drives much of the train-predict-infer loop in Figure \ref{algorithm}.

%This relation did not hold in the neural model. Regardless of the entity ratio, the model nearly always overpredicted entities. We explain this by pointing to the difference in semantics between the loss in a neural network, and the update in a single perceptron. In a perceptron, the semantics are clear: each update changes the weight vector and bias exactly according to the features in the instance. In a neural network, the non-linearities obscure the mechanism. It's never clear exactly how a particular update will change the parameters.

==> ilp.tex <==
\begin{figure}
\begin{align}
& \underset{\textbf{y}}{\text{max}} & & \sum_i^{|T|} C_0 y_{0i} + C_1 y_{1i} \label{objective}  \\
& \text{s.t.} & & \forall i,~ y_{0i} + y_{1i} = 1 \label{cantbothbeone} \\
& & & b-\delta \leq \sum_i y_{1i} / |T| \leq b+\delta \label{posconstraint} \\
%& & & \forall i,  \text{isPuncNum}(x_i), \sum_i y_{0i} \geq \epsilon |\text{PuncNum}|,  \\
& & & \forall i,~ x_i \in P,~ \sum_i y_{1i} \geq \xi |P|,  \label{pconstraint}\\
&&& \forall s \in S, \label{consista}\\
& && ~|s|a_s + \sum_{i \in s} y_{1i} \geq \alpha|s| \\
& && ~|s|b_s + \sum_{i \in s} y_{0i} \geq \alpha|s| \\
& && ~a_s+b_s=1 \label{consistb}
\end{align}
\caption{ILP for the inference step}
\label{binaryilp}
\end{figure}

\subsubsection{Constraints and Stopping Condition}

We encode our constraints with an Integer Linear Program (ILP), shown in Figure \ref{binaryilp}. Intuitively, the job of the inference step is to take predictions ($\hat{T}$) and use knowledge of the task to `fix' them. 

In the objective function (Eqn. \ref{objective}), token $i$ is represented by two indicator variables $y_{0i}$ and $y_{1i}$, representing negative and positive labels, respectively. Associated prediction scores $C_0$ and $C_1$ are from the classifier $\lambda$ in the last round of predictions. The first constraint (Eqn. \ref{cantbothbeone}) encodes the fact that an instance cannot be both an entity and a non-entity.

The second constraint (Eqn. \ref{posconstraint}) enforces the ratio of positive to total tokens in the corpus to match a required entity ratio. $|T|$ is the total number of tokens in the corpus. $b$ is the required entity ratio, which increases at each iteration. $\delta$ allows some flexibility, but is small.

The next constraint (Eqn. \ref{pconstraint}) encodes that instances in $P$ should be labeled as positive since they were manually labeled and are by definition trustworthy. We set $\xi \geq 0.99$.

%\swm{We could remove this constraint...} 
The last constraint (Eqns. \ref{consista}-\ref{consistb}) encodes the idea that identical surface forms should mostly, but not always, take the same label. $S$ is the sets of surface forms, and $\alpha$ is a parameter that allows us to soften this constraint. For example, the word `new' is sometimes an entity, as in `New Zealand', but mostly it is not. In our experiments, we use $\alpha=0.8$. The $a_s, b_s$ terms force the model to pick one or the other constraint. For example, if $a_s=1$, then the first constraint is trivially true, and only the second is enforced.

This framework is flexible in that more complex language- or task-specific constraints could be added. For simplicity, and because of the number of languages in our experiments, we use only a few constraints.

